Using LLMs for Analyzing AIS Data

Recent research in Large Language Models (LLMs), has had a profound impact across various fields, including mobility data science. This paper explores the and experiment with different approaches to using LLMs for analyzing AIS data. We propose a set of carefully designed queries to assess the reasoning capabilities of LLMs in this kind of tasks. Further, we experiment with four different methods: (1) using LLMs as a natural language interface to a spatial database, (2) reasoning on raw data, (3) reasoning on compressed trajectories, and (4) reasoning on semantic trajectories. We investigate the strengths and weaknesses for the four methods, and discuss the findings. The goal is to provide valuable insights for both researchers and practitioners on selecting the most appropriate LLM-based method depending on their specific data analysis objectives.

==> assets/data_model_Compressed.tex <==
\pgfplotstableread{               category  result_numeric  opp_result_numeric
            attribute           4.000               3.000
               fusion           2.500               6.500
individual-trajectory           3.000               4.000
     ship-interaction           0.875               3.125
}\modelCompressed

==> assets/data_model_PostGIS.tex <==
\pgfplotstableread{               category  result_numeric  opp_result_numeric
            attribute            5.50                1.50
               fusion            2.25                6.75
individual-trajectory            4.50                2.50
     ship-interaction            0.25                3.75
}\modelPostGIS

==> assets/data_model_Raw.tex <==
\pgfplotstableread{               category  result_numeric  opp_result_numeric
            attribute           4.000               3.000
               fusion           3.750               5.250
individual-trajectory           3.000               4.000
     ship-interaction           0.875               3.125
}\modelRaw

==> assets/data_model_Semantic.tex <==
\pgfplotstableread{               category  result_numeric  opp_result_numeric
            attribute           3.000               4.000
               fusion           2.500               6.500
individual-trajectory           3.000               4.000
     ship-interaction           0.875               3.125
}\modelSemantic

==> assets/data_size_100.tex <==
\pgfplotstableread{       model  result_numeric  opp_result_numeric
       Raw            7.25               18.75
Compressed            6.75               19.25
  Semantic            8.00               18.00
   PostGIS           14.00               13.00
}\sizeD

==> assets/data_size_20.tex <==
\pgfplotstableread{       model  result_numeric  opp_result_numeric
       Raw       12.500000           12.500000
Compressed       13.500000           12.500000
  Semantic       11.500000           13.500000
   PostGIS       14.333333           12.666667
}\sizeB

==> assets/data_size_5.tex <==
\pgfplotstableread{       model  result_numeric  opp_result_numeric
       Raw           19.00                8.00
Compressed           15.00               12.00
  Semantic           13.25               13.75
   PostGIS           14.00               13.00
}\sizeA

==> assets/data_size_50.tex <==
\pgfplotstableread{       model  result_numeric  opp_result_numeric
       Raw       10.583333           14.416667
Compressed        9.333333           15.666667
  Semantic        8.333333           16.666667
   PostGIS       12.500000           14.500000
}\sizeC

==> queries.tex <==
\begin{comment}
    
Hereunder are listed the queries used to evaluate the frameworks. 
\begin{enumerate}[label=\Alph*.]
  \item Attribute Queries:
    \begin{enumerate}[label=$\mathcal{Q}_\arabic*$:, leftmargin=1cm]
      \item What is the annual CO2 emission of ship $[MMSI]$?
      \item What is the CO2 emission of ship $[MMSI]$ per nautical mile ?
      \item What is the name of ship $[MMSI]$?
      \item What is the volume of displaced water of ship $[MMSI]$
      \item What is the IMO number for ship $[MMSI]$?
      \item How many ships are in the dataset?
      \item Assuming that the rectangle volume of a ship is a good approximation of its cargo capacity, which ship has the largest cargo capacity?
    \end{enumerate}
  \item Individual trajectories Queries:
    \begin{enumerate}[label=$\mathcal{Q}_{\arabic*}$:, resume, leftmargin=1cm]
      \item What is the maximum recorded speed of ship $[MMSI]$?
      \item Ship $[MMSI]$ is a ferry doing a round trip between two ports. It does it multiple times a day. What is the average single trip duration in minutes
      \item What is the total number of kilometers traveled by ship $[MMSI]$ for the day ?
      \item What is the average speed of ship $[MMSI]$ in kilometers per hour based on all moments where the ship was navigating ($SOG > 0.1$) ?
      \item What is the last known location of ship $[MMSI]$?
      \item What is the average waiting time for ship $[MMSI]$ at anchorage?
      \item For ferry $[MMSI]$, how many round trips did it complete ?
    \end{enumerate}
  \item Ship interactions Queries:
    \begin{enumerate}[label=$\mathcal{Q}_{\arabic*}$:, resume, leftmargin=1cm]
      \item Which other ships did ship $[MMSI]$ get close to $(< 500m)$ during its trip?
      \item Identify clusters of ships traveling together
      \item Which ships are ferry (always doing th same roundtrip) based on their navigation pattern?
    \end{enumerate}
  \item Fusion Queries:
    \begin{enumerate}[label=$\mathcal{Q}_{\arabic*}$:, resume, leftmargin=1cm]
      \item How long did ship $[MMSI]$ stayed at sea during the day (was not close or in a port) ?
      \item Which ship consumed most fuel between 15:00 and 16:00 on 2024-11-20?
      \item What is the average trip length from port Skagen to port Aarhus?
      \item Hypothetically, could ship $[MMSI]$ navigate through the Suez canal?
      \item Based on the travel distance of each ship for the day, and leveraging their respective fuel consumption, which ship polluted the most?
      \item Identify the ship with the best fuel efficiency (CO2 per nautical mile).
      \item What is the CO2 emission for one trip from Aarhus to Skagen for ship $[MMSI]$?
      \item Which is the most visited port for the day in terms of number of different boats that visited it?
      \item Where any ships in the dataset at risk of collision?
      \item Which ship did not go to sea today?
    \end{enumerate}
\end{enumerate}


\end{comment}
